PRISM (Polarized Radiation Imaging and Spectroscopy Mission): An Extended White Paper

PRISM (Polarized Radiation Imaging and Spectroscopy Mission) was proposed to ESA in May 2013 as a large-class mission for investigating within the framework of the ESA Cosmic Vision program a set of important scientific questions that require high resolution, high sensitivity, full-sky observations of the sky emission at wavelengths ranging from millimeter-wave to the far-infrared. PRISM's main objective is to explore the distant universe, probing cosmic history from very early times until now as well as the structures, distribution of matter, and velocity flows throughout our Hubble volume. PRISM will survey the full sky in a large number of frequency bands in both intensity and polarization and will measure the absolute spectrum of sky emission more than three orders of magnitude better than COBE FIRAS. The aim of this Extended White Paper is to provide a more detailed overview of the highlights of the new science that will be made possible by PRISM

==> abstract-prism.tex <==
{\small 

\noindent 
\mission\ (Polarized Radiation Imaging and Spectroscopy Mission) was proposed to ESA in May 2013 
as a large-class mission for investigating within the framework of the ESA Cosmic Vision 
program a set of important scientific questions that require high resolution, high sensitivity, full-sky 
observations of the sky emission
at wavelengths ranging from millimeter-wave to the far-infrared.
\mission's main objective is to explore the distant universe, probing cosmic 
history from very early times until now as well as the structures, distribution of 
matter, and velocity flows throughout our Hubble volume. \mission\  will 
survey the full sky in a large number of frequency bands in both 
intensity and polarization and will measure the absolute spectrum of sky emission more than 
three orders of magnitude better than {\it COBE} FIRAS. The data obtained will allow us
to precisely measure the absolute sky brightness and polarization of all the components of the
sky emission in the observed frequency range,
separating the primordial and extragalactic components cleanly from the galactic and zodiacal light emissions.
The aim of this Extended White Paper is to provide a more detailed overview of the highlights 
of the new science that will be made possible by \mission, which include: (1) the ultimate 
galaxy cluster survey using the Sunyaev-Zeldovich (SZ) effect, detecting approximately $10^6$ 
clusters extending to large redshift, including a characterization of the gas temperature of 
the brightest ones (through the relativistic corrections to the classic SZ template) as well 
as a peculiar velocity survey using the kinetic SZ effect that comprises our entire Hubble 
volume; (2) a detailed characterization of the properties and evolution of dusty galaxies, where 
the most of the star formation in the universe took place, the faintest population of which 
constitute the diffuse CIB (Cosmic Infrared Background); (3) a characterization of the B modes from 
primordial gravity waves generated during inflation and from gravitational lensing, as well 
as the ultimate search for primordial non-Gaussianity using CMB polarization, which is less 
contaminated by foregrounds on small scales than the temperature anisotropies; (4) a search 
for distortions from a perfect blackbody spectrum, which include some nearly certain signals 
and others that are more speculative but more informative; and (5) a study of the role of the 
magnetic field in star formation and its interaction with other components of the 
interstellar medium of our Galaxy. These are but a few of the highlights presented here 
along with a description of the proposed instrument.

}


==> authors-v2.tex <==
\noindent
{\small
\mission\ collaboration:
Philippe Andr\'e,
%
Carlo Baccigalupi, Anthony Banday, Domingos Barbosa, Belen Barreiro, James Bartlett, Nicola Bartolo, Elia Battistelli,
Richard Battye, George Bendo, Alain Beno\^it, Jean-Philippe Bernard, Marco Bersanelli, Matthieu B\'ethermin,
Pawel Bielewicz, Anna Bonaldi, Fran\c cois Bouchet, Fran\c cois Boulanger, Jan Brand, Martin Bucher, Carlo Burigana,
%
Zhen-Yi Cai, Philippe Camus, Francisco Casas, Viviana Casasola, Guillaume Castex, Anthony Challinor, Jens Chluba,
Gayoung Chon, Sergio Colafrancesco, Barbara Comis, Francesco Cuttaia,
%
Giuseppe D'Alessandro, Antonio Da Silva, Richard Davis, Miguel de Avillez, Paolo de~Bernardis, Marco de~Petris, Adriano de~Rosa,
Gianfranco de~Zotti, Jacques Delabrouille, Fran\c cois-Xavier D\'esert, Clive Dickinson, Jose Maria Diego, Joanna Dunkley,
%
Torsten En{\ss}lin, Josquin Errard,
%
Edith Falgarone, Pedro Ferreira, Katia Ferri\`ere, Fabio Finelli, Andrew Fletcher, Pablo Fosalba, Gary Fuller,
%
Silvia Galli, Ken Ganga, Juan Garc\'ia-Bellido, Adnan Ghribi, Martin Giard, Yannick Giraud-H\'eraud,
Joaquin Gonzalez-Nuevo, Keith Grainge, Alessandro Gruppuso,
%
Alex Hall, Jean-Christophe Hamilton, Marijke Haverkorn, Carlos Hernandez-Monte\-agudo, Diego Herranz,
%
Mark Jackson, Andrew Jaffe,
%
Rishi Khatri, Martin Kunz,
%
Luca Lamagna, Massimiliano Lattanzi, Paddy Leahy, Julien Lesgourgues, Michele Liguori, Elisabetta Liuzzo, Marcos Lopez-Caniego,
%
Juan Macias-Perez, Bruno Maffei, Davide Maino, Anna Mangilli,
Enrique Martinez-Gonzalez, Carlos Martins, Silvia Masi,
Marcella Massardi, Sabino Matarrese, Alessandro Melchiorri,
Jean-Baptiste Melin, Aniello Mennella, Arturo Mignano, Marc-Antoine Miville-Desch\^enes,
Alessandro Monfardini, Anthony Murphy,
%
Pavel Naselsky, Federico Nati, Paolo Natoli, Mattia Negrello, Fabio Noviello,
%
Cr\'eidhe O'Sullivan,
%
Francesco Paci, Luca Pagano, Rosita Paladino, Nathalie Palanque-Delabrouille, Daniela Paoletti, Hiranya Peiris, Francesca Perrotta,
Francesco Piacentini, Michel Piat, Lucio Piccirillo, Giampaolo Pisano, Gianluca Polenta, Agnieszka Pollo, Nicolas Ponthieu,
%
Mathieu Remazeilles, Sara Ricciardi, Matthieu Roman, Cyrille Rosset, Jose-Alberto Rubino-Martin,
%
Maria Salatino, Alessandro Schillaci, Paul Shellard, Joseph Silk, Alexei Starobinsky, Radek Stompor, Rashid Sunyaev,
%
Andrea Tartari, Luca Terenzi, Luigi Toffolatti, Maurizio Tomasi, Neil Trappe, Matthieu Tristram, Tiziana Trombetti, Marco Tucci,
%
Rien Van de Weijgaert, Bartjan Van~Tent, Licia Verde, Patricio Vielva,
%
Ben Wandelt, Robert Watson, Stafford Withington
}


==> supporters-v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{5mm}
\noindent
{\Large \bf \textit{\textbf{PRISM}}  Supporters}
\vspace{2mm}


\noindent
{\baselineskip=3pt 
As a result of 
the highly successful ESA Planck and Herschel missions, Europe has acquired considerable
scientific and technical expertise in the scientifically fruitful and strategic field of microwave and far-infrared
observations and trained 
a new generation of young European astronomers 
in this area.
The science themes outlined 
in this proposal are the logical next step
that will allow ESA to capitalize on these strengths. 
A list of supporters can be found at the following website:

\vskip 3pt

\textcolor{blue}{\large 
\url{http://www.prism-mission.org}
}

\vskip 3pt

\noindent
Scientists who believe that ESA should pursue 
as part of its programme the science themes presented in this White Paper are strongly encouraged to visit the website and to sign on as 
supporters.

}


